Verifying the Unknown: Correct-by-Design Control Synthesis for Networks of Stochastic Uncertain Systems

In this paper, we present an approach for designing correct-by-design controllers for cyber-physical systems composed of multiple dynamically interconnected uncertain systems. We consider networked discrete-time uncertain nonlinear systems with additive stochastic noise and model parametric uncertainty. Such settings arise when multiple systems interact in an uncertain environment and only observational data is available. We address two limitations of existing approaches for formal synthesis of controllers for networks of uncertain systems satisfying complex temporal specifications. Firstly, whilst existing approaches rely on the stochasticity to be Gaussian, the heterogeneous nature of composed systems typically yields a more complex stochastic behavior. Secondly, exact models of the systems involved are generally not available or difficult to acquire. To address these challenges, we show how abstraction-based control synthesis for uncertain systems based on sub-probability couplings can be extended to networked systems. We design controllers based on parameter uncertainty sets identified from observational data and approximate possibly arbitrary noise distributions using Gaussian mixture models whilst quantifying the incurred stochastic coupling. Finally, we demonstrate the effectiveness of our approach on a nonlinear package delivery case study with a complex specification, and a platoon of cars.

==> case_studies.tex <==
Platoon of two cars:
Real system is subject to drag and mass deviation impacting the change of velocities:
\begin{equation*}
	\begin{bmatrix}x_1^+\\v_1^+\\x_2^+\\v_2^+\\d^+\end{bmatrix} = \begin{bmatrix}1&\tau&0&0&0\\0&\theta_1&0&0&0\\0&0&1&\tau&0\\0&0&0&\theta_2&0\\0&\tau&0&-\tau&1\end{bmatrix}\begin{bmatrix}x_1\\v_1\\x_2\\v_2\\d\end{bmatrix}
	+\begin{bmatrix}0&0\\\tau\theta_3&0\\0&0\\0&\tau\theta_4\\0&0\end{bmatrix}\begin{bmatrix}u_1\\u_2\end{bmatrix} +\begin{bmatrix}0&0\\1&0\\0&0\\0&1\\0&0\end{bmatrix}w,
\end{equation*}
where the control inputs $u_1,u_2$ are the acceleration of the individual cars and $y=x$.
We retrieve the dynamics of the individual subsystems as
\begin{equation*}
	\begin{bmatrix}x_1^+\\v_1^+\\d^+\end{bmatrix} = \begin{bmatrix}1&\tau&0\\0&\theta_1&0\\0&\tau&1\end{bmatrix}\begin{bmatrix}x_1\\v_1\\d\end{bmatrix}
	+ \begin{bmatrix}0\\\tau\theta_3\\0\end{bmatrix}u_1
	+\begin{bmatrix}0\\1\\0\end{bmatrix}w_1
	\red{+\begin{bmatrix}0\\0\\-\tau\end{bmatrix}v_2},
\end{equation*}
and
\begin{equation*}
	\begin{bmatrix}x_2^+\\v_2^+\\d^+\end{bmatrix} = \begin{bmatrix}1&\tau&0\\0&\theta_2&0\\0&-\tau&1\end{bmatrix}\begin{bmatrix}x_2\\v_2\\d\end{bmatrix}
	+ \begin{bmatrix}0\\\tau\theta_4\\0\end{bmatrix}u_2
	+\begin{bmatrix}0\\1\\0\end{bmatrix}w_2
	\red{+\begin{bmatrix}0\\0\\\tau\end{bmatrix}v_1}.
\end{equation*}
Hence we get
\begin{align*}
	&G_1(\theta) = C_1\begin{bmatrix} B_1(\theta) & A_1B_1(\theta) & \ldots & [A_1(\theta)]^{T-2}B_1(\theta) \end{bmatrix} \in \R^{p\times m(T-1)}\\
	&= \begin{bmatrix} 
		0 & \tau^2\theta_3 & \tau^2\theta_3+\tau^2\theta_1\theta_3 
		%		& \tau^2\theta_3+\tau^2\theta_1\theta_3+\tau^2\theta_1^2\theta_3 
		& \ldots \\
		\tau\theta_3 & \tau\theta_1\theta_3 & \tau\theta_1^2\theta_3 
		%		& \tau\theta_1^3\theta_3 
		& \ldots \\
		0 & \tau^2\theta_3 & \tau^2\theta_1\theta_3+\tau^2\theta_3 
		%		& \tau^2\theta_1^2\theta_3+\tau^2\theta_1\theta_3+\tau^2\theta_3 
		& \ldots
	\end{bmatrix},
\end{align*}
and $G_2(\theta)$ analogously. \Oliver{Could also just look at G over first two rows/state variables.}
With unknown true values $\theta^\ast_1=0.9, \theta^\ast_2=0.7, \theta^\ast_3=0.9, \theta^\ast_4=0.7$.
With nominal values $\theta_1=1, \theta_2=1, \theta_3=1, \theta_4=1$.
Identified estimate $\hat\theta$ from first and second column of $G_1(\theta), G_2(\theta)$. Because the last state variable is decoupled from the external input we can not use it for parameter estimation.

The confidence set can be derived as follows (omitting index for subsystem): \Oliver{First two states only.}
\begin{align*}
	\Phi &\geq \norm{\hat G-G(\theta)} \\
	&= \norm{C[\hat B-B(\theta), \hat B\hat A-B(\theta)A(\theta),\ldots]}\\
	&= \norm{\begin{bmatrix} 
			0 & \tau^2(\hat\theta_3-\theta_3) & \ldots \\
			\tau(\hat\theta_3-\theta_3) & \tau(\hat\theta_1\hat\theta_3-\theta_1\theta_3) & \ldots
	\end{bmatrix}}\\
	&= \max_{\norm{\lambda}=1}\norm{\lambda_1\tau(\hat\theta_3-\theta_3) + \lambda_2[\tau^2(\hat\theta_3-\theta_3)+\tau(\hat\theta_1\hat\theta_3-\theta_1\theta_3)+\ldots]}\\
	&\geq \max_{\abs{\lambda_1+\lambda_2}=1}\norm{\lambda_1\underbrace{\tau(\hat\theta_3-\theta_3)}_{a(\theta,\hat\theta)} + \lambda_2\underbrace{[\tau^2(\hat\theta_3-\theta_3)+\tau(\hat\theta_1\hat\theta_3-\theta_1\theta_3)]}_{b(\theta,\hat\theta)}}
\end{align*}
Therefore, we can write the confidence set of subsystem one as a function of the LS estimate:
\begin{equation*}
	\Theta(\hat\theta) := \left\lbrace (\theta_1,\theta_3)\in\R^{2\mathfrak{p}}\given\max_{\abs{\lambda_1+\lambda_2}=1}\abs{\lambda_1a(\theta,\hat\theta) + \lambda_2b(\theta,\hat\theta)}\leq\Phi \right\rbrace.
\end{equation*}

\color{red}
For $\delta$ we get the following optimization problem:
\begin{align*}
	\delta_1(z_1, \hat\theta) = &\max_{\theta} \left\lbrace 1-2\cdot\cdf{-\frac{1}{2}\abs{x_{k,2}(\theta_1-\hat\theta_1)+\tau u_k(\theta_3-\hat\theta_3)}}\right\rbrace\\
	\text{s.t.}\quad &\abs{\lambda_1+\lambda_2}=1\\
	& \abs{\lambda_1\tau(\theta_3-\hat\theta_3)+\lambda_2[\tau^2(\theta_3-\hat\theta_3)+\tau(\theta_1\theta_3-\hat\theta_1\hat\theta_3)]}\leq\Phi
\end{align*}

==> composed_system_diagram.tex <==
\begin{figure}
	\centering
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
		%uncomment if require: \path (0,216); %set diagram left start at 0, and has height of 216
		
		%% System 1
		%Rounded Rect [id:dp22217799131680738] 
		\draw  [fill=grayfilling] (40,51) .. controls (40,44.92) and (44.92,40) .. (51,40) -- (84,40) .. controls (90.08,40) and (95,44.92) .. (95,51) -- (95,84) .. controls (95,90.08) and (90.08,95) .. (84,95) -- (51,95) .. controls (44.92,95) and (40,90.08) .. (40,84) -- cycle ;
		%Straight Lines [id:da08273469517536802] 
		\draw    (0,55) -- (38,55) ;
		\draw [shift={(40,55)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da7286474312267406] 
		\draw    (0,80) -- (31,80) -- (37.5,80) ;
		\draw [shift={(39.5,80)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da8497687026000231] 
		\draw    (68.5,0) -- (68.5,38) ;
		\draw [shift={(68.5,40)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da4118975490556376] 
		\draw    (0,80) -- (0,135) ;
		%Straight Lines [id:da8937728440260815] 
		\draw    (134.5,80) -- (135,135) ;
		%Straight Lines [id:da8764463118163162] 
		\draw    (95,55) -- (133,55) ;
		\draw [shift={(135,55)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da9345959359825047] 
		\draw    (95,80) -- (126,80) -- (134.5,80) ;
		
		%% System 2
		%Rounded Rect [id:dp649392069232241] 
		\draw  [fill=grayfilling] (40,131) .. controls (40,124.92) and (44.92,120) .. (51,120) -- (84,120) .. controls (90.08,120) and (95,124.92) .. (95,131) -- (95,164) .. controls (95,170.08) and (90.08,175) .. (84,175) -- (51,175) .. controls (44.92,175) and (40,170.08) .. (40,164) -- cycle ;
		%Straight Lines [id:da553449974709296] 
		\draw    (0,135) -- (40,135) ;
		%Straight Lines [id:da44280898997786755] 
		\draw    (2,160) -- (31,160) -- (39.5,160) ;
		\draw [shift={(0,160)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da004680366181214257] 
		\draw    (97,135) -- (135,135) ;
		\draw [shift={(95,135)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da4706598263906072] 
		\draw    (97,160) -- (126,160) -- (134.5,160) ;
		\draw [shift={(95,160)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da7775849255902443] 
		\draw    (68.5,177) -- (68.5,215) ;
		\draw [shift={(68.5,175)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		
		% Text Node
		\draw (2+1,58.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{12}$};
		% Text Node
		\draw (2+1,33.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{11}$};
		% Text Node
		\draw (97+1,58.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{12}$};
		% Text Node
		\draw (97+1,33.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{11}$};
		% Text Node
		\draw (13+1,138.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{22}$};
		% Text Node
		\draw (13+1,113.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{21}$};
		% Text Node
		\draw (108+1,138.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{22}$};
		% Text Node
		\draw (108+1,113.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{21}$};
		% Text Node
		\draw (45+1,8.4+2.5) node [anchor=north west][inner sep=0.75pt]    {$w_{1}$};
		% Text Node
		\draw (45+1,189.4+2.5) node [anchor=north west][inner sep=0.75pt]    {$w_{2}$};
		% Text Node
		\draw (55.5+1,57.4+2.5+1) node [anchor=north west][inner sep=0.75pt]    {$\M_{1}(\theta_1)$};
		% Text Node
		\draw (55.5+1,137.4+2.5+1) node [anchor=north west][inner sep=0.75pt]    {$\M_{2}(\theta_2)$};
	\end{tikzpicture}
	\caption{Interconnection of two subsystems}
	\label{fig:interconnected_system}
\end{figure}

==> compositional_old.tex <==
% !TEX root = main.tex
\begin{comment}
\color{gray}
\section{Compositional approach for sub-probability couplings of subsystems}
%\begin{quote}
%	"The abstraction framework is based on the notion of $\delta$-lifted relations, using which one can quantify the distance in probability between the interconnected gMDPs and that of their abstractions." \cite{lavaei2021compositional}
%\end{quote}
\Oliver{Insert short introduction with reference to \cite{lavaei2021compositional}.}\\
In the following, we drop the index $k$ on the time series $x_k,u_k$ for brevity.
Consider multiple interconnected gMDPs $\M_i$, $i=1,\ldots,N$, with unknown parameters $\theta_i\in\Theta_i$, respectively:
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= f_i(x_i,(u_i,v_i);\theta_i)+ R_i w_i\\
		y_i &= h_i(x_i),
	\end{array} \right.\label{eq:nonlinear_sys_subsys}
\end{align}
where $v_i$ denotes the internal inputs of subsystem $i$.
The nominal models are given as
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= \hat f_i(\hat x_i, (\hat u_i, \hat v_i);\theta^0_i)+ R_i\hat w_i\\
		\hat y_i &=  \hat h_i( \hat x_i).
	\end{array} \right.\label{eq:nonlinear_nom_subsys}
\end{align}
Note that the outputs $y_{ii}$, where $y_i:=[y_{i1},\ldots,y_{iN}]\T$, are external outputs, while $y_{ij}$ with $i\neq j$ are used internally to connect the individual subsystems to one another.

In the following, we assume that for all subsystems $i=1,\ldots,N$ we have \mbox{$\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$} and derive conditions so that \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\Mh$ and $\M$ are the interconnections of their respective subsystems. In the following, we formalize these concepts mathematically. First, we extend the definition of an SSR as stated in Def.~\ref{def:subsim} to subsystems.
\begin{definition}[SSR for subsystems]\label{def:ssr_subsys}
%	\Oliver{Replacement for Def.~3.2 in \cite{lavaei2021compositional}.}
	Consider two gMDPs
	$\M\!=\!(\X,x_0,\A\times\V, \Tr, h, \Y)$ and $\Mh\!=\!(\Xh,\xh{0},\Ah\times\Vh, \Trh, \hat h,  \Y)$, measurable relations $\R_{x}\subset \Xh\times\X$ and \Oliver{$\R_{\iin{}}\subset \Vh\times\V$}, and an interface function \(\InF :\Xh\times\X\times\Ah \rightarrow \A\). If there exists a sub-probability kernel  $\Wt(\cdot|\xh{},x, \Oliver{(\uh{}, \hat v, v)})$
such that
\begin{itemize}\itemsep=0pt
	\item[(a)] $(\hat x_{0}, x_{0})\in \R_{x}$;
	\item[(b)] for all $(\hat x,x)\in\R_{x}$, all $(\hat v,v)\in\R_{\iin{}}$, and $\ach{}\in \Ah$, $\Wt(\cdot|\xh{},x, \Oliver{(\uh{}, \hat v, v)})$ is a sub-probability coupling  of $\hat \Tr(\cdot|\hat x,\Oliver{(\uh{}, \hat v)})$ and $\Tr(\cdot|x,\Oliver{(\InF, v)})$ over $\R_{x}$ with respect to $\delta$ (c.f. Def.~\ref{def:submeasure_lifting}),
	\item[(c)] $\forall (\hat x,x)\in\R_{x}: \mathbf d_\Y(\hat h(\hat x),h(x)) \leq \varepsilon$,
\end{itemize}
then $\Mh$ is in an $(\varepsilon,\delta)$-SSR with $\M$  that is denoted as \mbox{$\Mh\preceq^{\delta}_\eps\M$}.
\end{definition}

%\begin{definition}[\bfseries Closeness for a composed system]\label{thm:closeness_composition}
%	\Oliver{Replacement for Thm.~3.5 in \cite{lavaei2021compositional}. Necessary?}
%\end{definition}
Let $\M_i\!=\!(\X_i,x^0_i,\A_i\times\V_i, \Tr_i, h_i, \Y_i)$ be a gMDP.
We can partition the internal input and output of $\M_i$ as
\begin{equation}\label{eq:partion_inout}
	v_i = [v_{i1}\T;\ldots;v_{i(i-1)}\T;v_{i(i+1)}\T;\ldots;v_{iN}\T], \quad i=1,\ldots,N,
\end{equation}
and the output space and function such that
\begin{equation}\label{eq:partion_infcn}
	h_i(x_i) = [h_{i1}\T(x_i);\ldots;h_{iN}\T(x_i)], \quad \Y_i=[\Y_{i1};\ldots;\Y_{iN}].
\end{equation}
%\begin{equation*}
%	C_i = [c_{i1}\T;\ldots;c_{iN}\T], \quad \Y_i=\Oliver{\bigcup_{j=1}^{N}}\Y_{ij}. \Oliver{\text{ or product?}}
%\end{equation*}
Furthermore, we separate the internal outputs $y_{ij}$, where $i\neq j$, from the external ones, i.e., $y_{ii}$, by forming interconnection constraint maps $g_i$, which will facilitate the interconnection of multiple gMDPs by enforcing $v_{i}=g_{i}$:
\begin{align}
	\begin{split}\label{eq:interconnection_constraint_maps}
		g_i(x_1,\ldots,x_N):=[h_{1i}\T (x_1);\ldots;h_{(i-1)i}\T (x_{i-1});\\h_{(i+1)i}\T (x_{i+1});\ldots;h_{Ni}\T (x_N)].
	\end{split}
\end{align}
Next, we define the interconnection of multiple subsystems.

\begin{definition}[Interconnection of subsystems]\label{def:interconnection}
%	\Oliver{Replacement for Def.~4.1 in \cite{lavaei2021compositional}.}
	Consider $N\in\mathbb{N}_{\geq 1}$ gMDPs $\M_i\!=\!(\X_i,x^0_i,\A_i\times\V_i, \Tr_i, h_i, \Y_i)$, $i=1,\ldots,N$, with an input-output configuration which can be partitioned as in \eqref{eq:partion_inout}-\eqref{eq:partion_infcn}. Then, the \emph{interconnection} of subsystems $\M_i$ is a gMDP $\M\!=\!(\X,x^0,\A\times\V, \Tr, h, \Y)$, also denoted as $\Interc{\M_1,\ldots,\M_N}$, such that $\X=[\X_{1};\ldots;\X_{N}]$, $\U=[\U_{1};\ldots;\U_{N}]$, $\V=[\V_{1};\ldots;\V_{N}]$, $\Y=[\Y_{11};\ldots;\Y_{NN}]$, $h=[h_{11};\ldots;h_{NN}]$, with interconnection constraints
	\begin{equation}\label{eq:interconnection_constraints}
		\forall i,j=1\ldots,N,\, i\neq j:\, v_{ji}=y_{ij},\, \Y_{ij}\subseteq\V_{ji}.
	\end{equation}
	The kernel and initial distribution are given as $\Tr=\prod_{i=1}^{N}\Tr_{i}$ and $x^0=[x^0_{1};\ldots;x^0_{N}]$, respectively.
\end{definition}

In the next theorem we establish \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\M=\Interc{\M_1,\ldots,\M_N}$ and $\Mh=\Interc{\Mh_1,\ldots,\Mh_N}$, by induction from $\forall i=1,\ldots,N:\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$.

\begin{theorem}[\bfseries Induced compositional SSR]\label{thm:comp_induction}
%	\Oliver{Replacement for Thm.~4.3 in \cite{lavaei2021compositional}.}
	Consider $N\in\mathbb{N}_{\geq 1}$ gMDPs $\M_i(\theta_i)$, $i=1,\ldots,N$, forming an interconnected gMDP $\M(\theta)=\Interc{\M_1,\ldots,\M_N}$, with $\theta:=[\theta_1,\ldots,\theta_N]$. Suppose that there exist $N$ abstract gMDPs $\Mh_i$ independent of $\theta_i$, such that for all $i=1,\ldots,N$ $\Mh_i$ is in an $(\varepsilon_i, \delta_i)$-SSR with $\M_i(\theta_i)$ as defined in Def.~\ref{def:ssr_subsys} with corresponding relations $R_{x_i}$, $\R_{\iin{i}}$, and sub-probability coupling $\Wt_i$. If for all \red{$i,j=1,\ldots,N$ we have
	\begin{equation*}
		\forall (\hat x_j, x_j)\in\R_{x_j}: \, \left(\hat g_i(\hat x_1,\ldots,\hat x_N), g_i(x_1,\ldots,x_N)\right)\in\R_{\iin{i}},
	\end{equation*}
	}with interconnection constraint maps $\hat g_i$, $g_i$ as defined in \eqref{eq:interconnection_constraint_maps},
	then $\Mh=\mathscr{I}(\Mh_1,\ldots,\Mh_N)$ is in an \emph{induced compositional} $(\varepsilon, \delta)$-SSR with $\M(\theta)$ as defined in Def.~\ref{def:subsim} with a relation $\R$ given as 
	\begin{equation*}
		(\hat x, x)\in\R \Leftrightarrow \forall i=1,\ldots,N:\, (\hat x_i, x_i)\in\R_{x_i}
	\end{equation*}
	where $\hat x:=[\hat x_1;\ldots;\hat x_N]$ and $x:=[x_1;\ldots;x_N]$,
	and \Oliver{$\varepsilon=\sum_{i=1}^{N}\varepsilon_i$}, \Oliver{$\delta=1-\prod_{i=1}^{N}(1-\delta_i)$}. Furthermore, we obtain the sub-probability coupling \Oliver{$\Wt=\prod_{i=1}^{N}\Wt_{i}$} and the interface function \Oliver{$\InF=\prod_{i=1}^{N}\InF_{i}$}, substituting with the interconnection constraints in \eqref{eq:interconnection_constraints}.
\end{theorem}


\subsection{Linear subsystems}
Let us now look at the case where the overall system can be decomposed into multiple linear subsystems $\M_i$. 
Consider $N$ interconnected gMDPs, $i=1,\ldots,N$, i.e.,
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= A_i x_i+ B_i u_i+ D_i v_i+ R_i w_i+F_i \theta_i\\
		y_i &= C_i x_i,
	\end{array} \right.\label{eq:linear_sys_subsys}
\end{align}
and corresponding nominal models
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= A_i \hat x_i+  B_i \hat u_i+ D_i \hat v_i+ R_i\hat w_i\\
		\hat y_i &=  C_i \hat x_i.
	\end{array} \right.\label{eq:linear_nom_subsys}
\end{align}
%Note that the outputs $y_{ii}$, where $y_i:=[y_{i1},\ldots,y_{iN}]\T$, are external outputs, while $y_{ij}$ with $i\neq j$ are used internally to connect the individual subsystems to each other.
The transition kernels can consequently be written as
\begin{align*}
	\Tr_i(\dxp_i \given x_i, u_i, v_i) &= \mathcal N(\dxp_i|A_i x_i+ B_i u_i+ D_i v_i +F_i \theta_i, R_iR_i\T)\\
	\Trh_i(\dxhp_i \given \hat x_i, \hat u_i, \hat v_i) &= \mathcal N(\dxhp_i|A_i \hat x_i+ B_i \hat u_i+ D_i \hat v_i, R_iR_i\T).
\end{align*}

%\hrule
We choose the interface function $\ac{i}\sim\InF_i(\cdot|\hat x_i, x_i, \hat u_i):=\ach{i}$,
and the noise coupling $\hat w_i=w_i+R^{-1}_i F_i\theta_i$ to get the state mapping
\[ \xhp_i = \xp_i-A (x_i-\hat x_i)-B (\ac{i}-\ach{i})-D(v_i-\hat v_i), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_subsys}
	\xhp_i \sim \Refi_i(\cdot |\xh{i}, \x{i}, \xp_{i},\ach{i}) = \delta_{\xp_i-A x^\Delta_i-B u^\Delta_i-Dv^\Delta_i}(d\xhp_i),
\end{equation}
where $v^\Delta_i:=v_{i}-\hat v_{i}$.
To establish an SSR $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$, we select the relations
\begin{align}
	\R_{x_i}&:=\{ (\hat x_i,x_i)\in\Xh_i\times\X_i \given x_i=\hat x_i\}\label{eq:R_x}\\
	\R_{\iin{i}}&:=\{ (\hat v_i,v_i)\in\Vh_i\times\V_i \given v_i=\hat v_i\}.\label{eq:R_v}
\end{align}
Condition (a) of Def.~\ref{def:ssr_subsys} holds by setting the initial states $\hat x^{0}_i = x^{0}_i$. Condition (c) is satisfied with $\eps_i=0$ since both systems use the same output mapping. For condition (b), we define the sub-probability coupling $\Wt_i$ of $\hat \Tr_i(\cdot|\hat x_i,\ach{i})$ and $\Tr_i(\cdot|x_i,\InF_i)$ over $\R_{x_i}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_subsys}
		\Wt_i
		&=\del{d\xhp_i}{\xp_i}
		\min\{\mathcal N(d\xp_i|\Phi_i,R_iR_i\T),\\&\mathcal N(d\xp_i|\Phi_i-R^{-1}_i F_i\theta_i, R_iR_i\T)\},
	\end{split}
\end{align}
with $\Phi_i := A_i x_i+ B_i u_i+ D_i v_i+ F_i\theta_i$, that takes the minimum of two probability measures.

\begin{theorem}
	\label{thm:linear_subsys}
	For the linear models in \eqref{eq:linear_sys_subsys}-\eqref{eq:linear_nom_subsys}, we have that $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ with interface function $\ac{i} = \ach{i}$, relations \eqref{eq:R_x}-\eqref{eq:R_v}, and the sub-probability kernel \eqref{eq:subprobcoup_subsys}. The state mapping \eqref{eq:statemap_subsys} defines a valid control refinement with $\eps_i=0$ and
	\begin{equation}
		\label{eq:delta_subsys}
		\delta_i = \sup_{\theta_i\in\Theta_i}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\norm{R^{-1}_i F_i\theta_i}}\right\rbrace.
	\end{equation}
\end{theorem}

	
\subsection{\Oliver{Composed system}}
Now we connect two subsystems, $i\in\{1,2\}$, with $\iin{1}=y_2$ and $\iin{2}=y_1$ (i.e., with $\iinh{1}=\hat y_2$ and $\iinh{2}=\hat y_1$). For $x:=[x_1,x_2]\T\in\X$, $\hat x:=[\hat x_1,\hat x_2]\T\in\Xh$, $u:=[u_1,u_2]\T\in\A$, $\hat u:=[\hat u_1,\hat u_2]\T\in\Ah$, and $\theta:=[\theta_1,\theta_2]\T\in\Theta$ we find the compositional transition kernels for the interconnected gMDPs $\M(\theta)$ and $\Mh$, namely
\begin{align*}
	\Tr(\dxp \given x, u) &= \mathcal N(\dxp|\bar A x+ B u+F \theta, RR\T)\\
	\Trh(\dxhp \given \hat x, \hat u) &= \mathcal N(\dxhp|\bar A \hat x+ B \hat u, RR\T).
\end{align*}
%with $u=\hat u$, $x=\hat x$, and 
where $B:=\mathrm{diag}(B_1,B_2)$, $F:=\mathrm{diag}(F_1,F_2)$, $R:=\mathrm{diag}(R_1,R_2)$, and
\begin{align*}
	\bar A&:=\begin{bmatrix} A_1 & D_1C_2 \\ D_2C_1 & A_2 \end{bmatrix}.
\end{align*}

We get the state mapping
\[ \xhp = \xp-\bar A (x-\hat x)-B (\ac{}-\ach{}), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_comp}
	\xhp \sim \Refi(\cdot |\xh{}, \x{}, \xp{},\ach{}) = \delta_{\xp-\bar A x^\Delta-B u^\Delta}(d\xhp).
\end{equation}
To establish an SSR of the composed system, i.e., $\Mh\preceq^{\delta}_{\eps}\M(\theta)$, we select the relation
\begin{align}\label{eq:R_comp}
	\R_{x}&:=\{ (\hat x,x)\in\Xh\times\X \given x=\hat x\}
\end{align}
Condition (a) of Def.~\ref{def:subsim} holds by setting the initial states $\hat x^{0} = x^{0}$. Condition (c) is satisfied with $\eps=0$ since both compositional systems use the same output mapping, i.e., $C:=\mathrm{diag}(C_1,C_2)$. For condition (b), we define the sub-probability coupling $\Wt$ of $\hat \Tr(\cdot|\hat x,\ach{})$ and $\Tr(\cdot|x,\InF)$ over $\R_{x}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_comp}
		\Wt&=\del{d\xhp}{\xp} \min\{\mathcal N(d\xp|\Phi,RR\T),\\
		&\mathcal N(d\xp|\Phi-R^{-1}F\theta_, RR\T)\},
	\end{split}
\end{align}
with $\Phi := \bar A x+ B u+ F\theta$, that takes the minimum of two probability measures.

Now we want to establish a probabilistic relation after the composition using Thm.~\ref{thm:comp_induction}, which enables us to get guarantees on the closeness of the composed system and its abstraction using Thm.~\ref{thm:linear_subsys}.

%\subsection{\Oliver{Establishing probabilistic relations}}
%In this subsection, we derive the conditions under which $\Mh$ in \eqref{eq:linear_nom_subsys} is in an $(\varepsilon,\delta)$-SSR with $\M$ in \eqref{eq:linear_sys_subsys} with relations $\R_x$ and $\R_w$ as defined in \eqref{eq:R_x}-\eqref{eq:R_v}.

\begin{theorem}
	Consider $N\in\mathbb{N}_{\geq 1}$ linear subsystems \eqref{eq:linear_sys_subsys}-\eqref{eq:linear_nom_subsys}, where $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ for $i=1,\ldots,N$ with relations \eqref{eq:R_x}-\eqref{eq:R_v}, interface functions $u_i=\hat u_i$, and sub-probability kernels \eqref{eq:subprobcoup_subsys}.
	Let, $\M=\Interc{\M_1,\ldots,\M_N}$ and $\Mh=\Interc{\Mh_1,\ldots,\Mh_N}$ be the interconnections of these linear subsystems. Then Thm.~\ref{thm:comp_induction} holds, with relation $\R=\{ (\hat x,x)\in\Xh\times\X\given x=\hat x\}$, interface function $\ac{} = \ach{}$, and sub-probability kernel \eqref{eq:subprobcoup_comp}.
\end{theorem}
\begin{proof}
	It is trivial to show that the interconnection constraints in Thm.~\ref{thm:comp_induction} hold for this choice of $\R_{x_i},\R_{\iin{i}}$.
\end{proof}


%
%	\Oliver{
%		Using $\hat w:= \Gamma w+\offset$
%		\subsubsection{Def.~\ref{def:submeasure_lifting}(a)}\label{app:def_sub_a}
%		To prove that all considered distributions of \eqref{eq:subprobcoup_new} satisfy $\operatorname{supp}(\W)\subset\rel$ (c.f. Def.~\ref{def:submeasure_lifting}(a)), we first show $\forall z\in\Z: \W(\Xh\times\X)\geq 1-\delta$ and then $\forall z\in\Z: \W(\Xh\times\X) = \W(\R)$.
%		
%		
%		From Eq.~\eqref{eq:subprobcoup_new} we get for a fixed $z\in\Z$
%		\begin{align*}
%			&\W(\Xh\times\X) = \int_{\xhp\in\Xh} \int_{\xp\in\X} \int_{w} \W(\dxhp\times \dxp)\\
%			&= \int_{w} \int_{\xhp\in\Xh} \int_{\xp\in\X} \fhdel{\dxhp| \Gamma w+\offset} \fdel{\dxp| w; \theta} \\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}.
%		\end{align*}
%		Using definitions \eqref{eq:fdel_lin_new}-\eqref{eq:fhdel_lin_new} we rewrite to obtain
%		\begin{align*}
%			&\W(\Xh\times\X) = \int_{w} \int_{\xhp\in\Xh} \int_{\xp\in\X} \delta_{\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)}(\dxhp)\\
%			&\delta_{Ax_k+Bu_k+Rw+F\theta}(\dxp) \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&= \int_{w} \1(A x_k+B u_k+Rw+F\theta\in\X)\\& \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)\in\Xh)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}.
%		\end{align*}
%		Since $\forall z\in\Z,w\exists\xp\in\X: \xp = A x_k+B u_k+Rw+F\theta$ and $\forall z\in\Z,w\exists\xhp\in\Xh: \xhp = \hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)$, we get $\W(\Xh\times\X) = \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}$.
%		
%		
%		Similarly, we derive from \eqref{eq:subprobcoup_new}
%		\begin{align*}
%			&\W(\R) = \int_{(\xhp, \xp)\in\R} \int_{w} \W(\dxhp\times \dxp)\\
%			&= \int_{w} \int_{(\xhp, \xp)\in\R} \fhdel{\dxhp| \Gamma w+\offset} \fdel{\dxp| w; \theta} \\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&= \int_{w} \1((\hat A\hat x_k+\hat B\hat u_k+\Gamma w+\offset,\\&Ax_k+Bu_k+Rw+F\theta)\in\R)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\},
%			%	&= \int_{w} \int_{(\xhp, \xp)\in\R}  \delta_{f(\hat x_k,\hat u_k,w+\theta;\theta_0)}(\dxhp)\delta_{f(x_k,u_k,w;\theta)}(\dxp)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}\\\
%		\end{align*}
%		and get after simplifying using $\hat x_k=x_k$ and $\ach{k}=\ac{k}$
%		\begin{align*}
%			&\W(\R) = \1((\hat A-A)\hat x_k+(\hat B-B)\hat u_k+(\Gamma-R) w+\offset=F\theta)\\& \int_{w}  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\},
%		\end{align*}
%		yielding $\W(\R) = \W(\Xh\times\X)$ independent of $z$. This proves that \eqref{eq:subprobcoup_new} satisfies condition (a) of Def.~\ref{def:submeasure_lifting}.
%		
%		
%		CALCULATION OF DELTA SKIPPED:
%		\begin{equation*}
%			\delta(\xh{k},\ach{k}) = \sup_{\theta\in\Theta}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\Phi\norm{\offset(\xh{k},\ach{k},\theta)}}\right\rbrace
%		\end{equation*}
%		
%		\subsubsection{Def.~\ref{def:submeasure_lifting}(b)}\label{sec:proof_th3b_}
%		Prove $\forall z\in\Z,S \subset \hat \X:\W(S \times \X) \leq \hat t(S)$.
%		First, we consider the integral of the individual distributions of the transition kernel \eqref{eq:tr_hat_new} over $S$. For a fixed $z\in\Z$ we get
%		\begin{align}
%			\begin{split}\label{eq:transKernelTemp1_}
%				&\hat t(S) = \int_{\xhp\in S} \hat t(\dxhp) \\
%				&= \int_{\xhp\in S}  \int_{\hat w}\fhdel{\dxhp|\hat w}\mathcal N(d\hat w|0, I)\\
%				&=  \int_{\hat w} \int_{\xhp\in S} \delta_{\hat A\hat x_k+\hat B\hat u_k+\hat R\hat w}(\dxhp)\mathcal N(d\hat w|0, I)\\
%				&=  \int_{\hat w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat R\hat w \in S)\mathcal N(d\hat w|0, I).
%			\end{split}
%		\end{align}
%		We will use this equation later on. Next, from \eqref{eq:subprobcoup_new} we get
%		\begin{align*}
%			&\W(S \times \X) = \int_{\xhp\in S}  \int_{\xp\in \X}  \int_{w} \W(\dxhp \times \dxp)\\
%			&=  \int_{w}  \int_{\xp\in \X}  \fdel{\dxp| w; \theta} \int_{\xhp\in S} \fhdel{\dxhp| \Gamma w+\offset} \\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&=  \int_{w}  \int_{\xp\in \X} \delta_{Ax_k+Bu_k+Rw+F\theta}(\dxp)\\& \int_{\xhp\in S} \delta_{\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)}(\dxhp)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}\\
%			&=  \int_{w} \1(A x_k+B u_k+Rw+F\theta\in\X)\\& \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\Gamma w+\offset)\in S)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\Phi\theta, I)\}.
%		\end{align*}
%		Since $\forall z\in\Z,w \exists \xp\in \X: \xp = A x_k+B u_k+Rw+F\theta$, this integral can equivalently be written as
%		\begin{align*}
%			&\W(S \times \X) = \int_{w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\hat R w+\offset)\in S)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}\\
%			&= \int_{\hat w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(\hat R w+\offset)\in S)\\& \min\{ \frac{dw}{ \sqrt{(2\pi)^n \!\left| I \right| }}\exp\!\left[\!-\frac{1}{2}w\T\! I^{-1}\!w\!\right],\\& \frac{dw}{ \sqrt{(2\pi)^n \!\left| I \right| }}\exp\!\left[\!-\frac{1}{2}(w\!+\!\offset)\T\! I^{-1}\!(w\!+\!\offset)\!\right]\}\\
%			&= \int_{\hat w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat Rw\in S)\\& \min\{ \frac{dw}{ \sqrt{(2\pi)^n \!\left| \hat R\hat R\T \right| }}\exp\!\left[\!-\frac{1}{2}(w-\gamma)\T\! (\hat R\hat R\T)^{-1}\!(w-\gamma)\!\right],\\& \frac{dw}{ \sqrt{(2\pi)^n \!\left| \hat R\hat R\T \right| }}\exp\!\left[\!-\frac{1}{2}w\T\! (\hat R\hat R\T)^{-1}\!w\!\right]\}\\
%			&=\int_{w} \1(\hat A\hat x_k+\hat B\hat u_k+\hat w\in S)\\&  \min\{\mathcal N(dw|\offset,\hat R\hat R\T),\mathcal N(dw|0,\hat R\hat R\T )\}\\
%			&= \int_{\hat w}  \1(\hat A\hat x_k+\hat B\hat u_k+\hat R\hat w\in S)\\&  \min\left\lbrace \mathcal N(d\hat w|\offset,I), \mathcal N(d\hat w|0,I)\right\rbrace\\
%			&\leq \int_{\hat w}  \1(A\hat x_k+B\hat u_k+\hat R\hat w\in S) \mathcal N(d\hat w|0,I).
%		\end{align*}
%		Substituting Eq.~\eqref{eq:transKernelTemp1__new} yields $\forall z\in\Z:\W(S \times \X) \leq  \hat t(S)$,
%		concluding that \eqref{eq:subprobcoup_new} satisfies condition (b) of Def.~\ref{def:submeasure_lifting}.
%		
%		\subsubsection{Def.~\ref{def:submeasure_lifting}(c)}
%		Prove $\forall z\in\Z,S \subset \X:\W(\Xh \times S) \leq t(S)$.
%		Analogously to App.~\ref{sec:proof_th3b__new} we consider the integral of the individual distributions of the transition kernel \eqref{eq:tr_new} over $S$. For a fixed $z\in\Z$ we get
%		\begin{align}
%			\begin{split}\label{eq:transKernelTemp2_}
%				&t(S) = \int_{\xhp\in S}t(\dxp) \\
%				&= \int_{w} \1(Ax_k+Bu_k+Rw+F\theta\in S)\mathcal N(dw|0, I).
%			\end{split}
%		\end{align}
%		Next, using Eq.~\eqref{eq:subprobcoup_new} we get
%		\begin{align*}
%			&\W(\Xh \times S) = \int_{\xhp\in \Xh}  \int_{\xp\in S}  \int_{w} \W(\dxhp \times \dxp)\\
%			&=  \int_{w}  \1(\hat A\hat x_k+\hat B\hat u_k+\hat R(w+\theta)\in\Xh)\\ &\1(Ax_k+Bu_k+w+\theta\in S)\\&  \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}.
%		\end{align*}
%		Since $\forall z\in\Z,w \exists \xhp\in \Xh: \xhp = \hat A\hat x_k+\hat B\hat u_k+\hat R(w+\theta)$, it follows that
%		\begin{align*}
%			&\W(\Xh \times S) = \int_{w} \1(Ax_k+Bu_k+Rw+F\theta\in S)\\& \min\{\mathcal N(dw|0,I),\mathcal N(dw|-\theta, I)\}\\
%			&\leq \int_{w} \1(Ax_k+Bu_k+Rw+F\theta\in S) \mathcal N(dw|0,I)\\
%			&= t(S),
%		\end{align*}
%		yielding $\forall z\in\Z:\W(\Xh \times S) \leq  t(S)$,
%		therefore concluding that \eqref{eq:subprobcoup_new} satisfies condition (c) of Def.~\ref{def:submeasure_lifting}. Hence, having proven that \eqref{eq:subprobcoup_new} satisfies all conditions of Def.~\ref{def:submeasure_lifting}, \eqref{eq:subprobcoup_new} is a valid sub-probability coupling.
%		
%		\subsubsection{Def.~\ref{def:validrefinement}}
%		From the state mapping $\hat R\hat w=Rw+F\theta$, i.e., $\xhp- \hat A\hat x-\hat B\hat u=\xp-Ax-Bu$, we find a composed probability measure using Eq.~\ref{eq:compprobmeas_new}:
%		\begin{align*}
%			&\bar{\Refi} = \delta_{\xp-Ax-Bu+\hat A\hat x+\hat B\hat u}(d\xhp) \Tr(\dxp|x,\InF(\ac{k}|\hat x_k, x_k, \hat u_k))\\
%			&= \delta_{\xp-Ax-Bu+\hat A\hat x+\hat B\hat u}(d\xhp) \int_w \fdel{\dxp|w;\theta} \mathcal N(dw|0, I)\\
%			&= \int_w \delta_{A\hat x_k+B\hat u_k+F\theta+Rw)}(d\xhp)  \fdel{\dxp|w;\theta} \mathcal N(dw|0, I)\\
%			&= \int_w \fhdel{\dxhp|\hat R^{-1}(F\theta+Rw)} \fdel{\dxp|w;\theta} \mathcal N(dw|0, I)\\
%			&= \int_w \int_{\hat w} \fhdel{\dxhp|\hat w} \fdel{\dxp|w;\theta}  \delta_{\hat R^{-1}(F\theta+Rw)}(d\hat w) \mathcal N(dw|0, I),
%		\end{align*}
%		which upper-bounds the sub-probability coupling $\Wt$ and therefore proves that Eq.~\eqref{eq:statemap} is a valid control refinement as formalized in Def.~\ref{def:validrefinement}. 
%		This concludes the proof of Thm.~\ref{thm:linear}.
%	}







\color{black}
\end{comment}

\subsection{Simulation relations for compositional systems}
%\section{Compositional approach for sub-probability couplings of two subsystems}
%\Oliver{Insert short introduction with reference to .}\\

The applicability of abstraction-based verification and synthesis methods is strongly limited by the dimensionality of the targeted system \cite{lavaei2021automated}. Therefore, one stream of research is pursuing strategies for exploiting the structure of a system to relieve the computational burden. One such strategy is to partition a system into a set of subsystems which together form a \emph{compositional system} \cite{lavaei2021compositional}. After establishing probabilistic closeness guarantees between the individual subsystems and their abstracted counterparts in the form of simulation relations, compositional approaches enable us to substitute the problem of synthesizing a monolithic controller on the whole system by computing local controllers for each low-dimensional subsystem. It can be shown that the robustness guarantees are inherited by the interconnected system. \red{Note that this is only possible if (a) the specification can likewise be partitioned as well or (b) the subsystems are identical.} \Oliver{Otherwise state variables have to be passed through and hence increase the state dimension?!}
\Oliver{In the previous papers for the synthesis of a local controller on a subsystem they always take the worst-case considering the whole specified state-space for the state variables of the other subsystems routed to the subsystem in scope. Also, isn't going to be as good as globally/monolithic optimal controller.} \Oliver{The compositional approach in its native form is only powerful if you can almost ignore the other subsystems. Which defeats the purpose in a CPS!?}

In this section, we show how our definition of simulation relations for parametric systems can be combined with the results for compositional systems in \cite{lavaei2021compositional}. In \cite{lavaei2021compositional}, the authors are following the dissipativity approach to compositionality, i.e., the error of the composed system is additive in the errors of the underlying subsystems (see, e.g., \cite{Lavaei2020smallgain}).
%\Oliver{Alternative would be Small-Gain approach (less conservative).)}

In the following, we drop the index $k$ on the time series $x_k,u_k$ for brevity.
Although the compositional approach is scalable to any number of subsystems, we consider only two subsystems here, with the results being easily extendable to more general settings.

Consider two gMDPs $\M_1(\theta_1)$, $\M_2(\theta_2)$ with unknown parameters $\theta_1\in\Theta_1\subset\mathbb{R}^{\mathfrak{p}}$, $\theta_2\in\Theta_2\subset\mathbb{R}^{\mathfrak{p}}$, respectively:
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= f_i(x_i,u_i;\theta_i)+ B_{w,i} w_i\\
		y_i &= h_i(x_i),
	\end{array} \right.\label{eq:nonlinear_sys_subsys_two}
\end{align}
%\Oliver{Replace $\Z$ definition here bc used in appendix. Should be $\underline{\mathbb{Y}}$.}
described by states $x_i\in\X_i$ and
where the inputs and outputs can be partitioned as follows:
\begin{equation}\label{eq:input_output_partitioning}
	u_i:=[u_{i1},u_{i2}]\T,\quad y_i:=[y_{i1},y_{i2}]\T,
\end{equation}
where $u_{ij}\in \U_{ij},\forall j\neq i$ denotes the $j$-th internal input of subsystem $i$,
and $y_{ij}\in\Y_{ij},\forall j\neq i$ the $j$-th internal output of subsystem $i$. 
The external inputs and outputs are $u_{ii}\in \U_{ii}$ and $y_{ii}\in \Y_{ii}$ for all $i=1,2$, respectively.
Note that the output function can be decomposed as $h_i=\left[h_{i1};h_{i2}\right]$ such that $y_{ij}=h_{ij}$ for all $i,j=1,2$. 
Furthermore, we recover $\U_i=\prod_{j}\U_{ij}$ and $\Y_i=\prod_{j}\Y_{ij}$.
%The two subsystems are connected by setting $u_{12}=y_{21}$ and $u_{21}=y_{12}$.
The corresponding nominal models are given as
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= \hat f_i(\hat x_i, \hat u_i;\theta^0_i)+ B_{w,i}\hat w_i\\
		\hat y_i &=  \hat h_i( \hat x_i),
	\end{array} \right.\label{eq:nonlinear_nom_subsys_two}
\end{align}
with similar partitioning, $\hat x_i\in\Xh_i$, $\forall i,j=1,2:\hat u_{ij}\in\Uh_{ij},\hat y_{ij}\in\Yh_{ij}$, $\forall i=1,2:\Yh_{ii}=\Y_{ii}$, $\Uh_i=\prod_{j}\Uh_{ij}$, and $\Yh_i=\prod_{j}\Yh_{ij}$. \red{We assume that $B_{w,i}$ is invertible.}
%The output $y_1$ of gMDP $\M_1$ consists of an external output $y_{11}$ and an internal output $y_{12}$, latter of which is used internally to connect $\M_1$ to $\M_2$ by setting $\iin{2}\equiv y_{12}$. We get $y_1:=[y_{11};y_{12}]$. The output of gMDPs $\M_2,\Mh_1,\Mh_2$ are defined analogously.

In the following, we assume that for both $i=1,2$ we have \mbox{$\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$} and derive conditions so that \mbox{$\Mh\preceq^{\delta}_\eps\M(\theta)$}, where $\Mh$ and $\M(\theta)$ are the interconnections of their respective subsystems. Next, we formalize these concepts mathematically. First, we extend the definition of an SSR as stated in Def.~\ref{def:subsim} to subsystems.

\hrule
%\begin{definition}[SSR for a subsystem]\label{def:ssr_subsys_two}
%	%	\Oliver{Replacement for Def.~3.2 in \cite{lavaei2021compositional}.}
%	Consider two gMDPs
%	$\M_i\!=\!(\X_i,x_{0,i},\U_i, \Tr_i, h_i, \Y_i)$ and $\Mh_i\!=\!(\Xh_i,\xh{0,i},\Uh_i, \Trh_i, \hat h_i,  \Y_i)$, measurable relations $\R_{x_i}\subset \Xh_i\times\X_i$ and $\R_{u_{i}}\subset \Uh_{ij}\times\U_{ij},\forall j\neq i$, and an interface function \(\InF_i :\Xh_i\times\X_i\times\Uh_{ii} \rightarrow\U_{ii}\). If there exists a sub-probability kernel  $\Wt_i(\cdot|\xh{i},x_i,\red{\uh{i}})$
%	such that
%	\begin{itemize}\itemsep=0pt
%		\item[(a)] $(\hat x_{0,i}, x_{0,i})\in \R_{x_i}$;
%		\item[(b)] for all $(\hat x_i,x_i)\in\R_{x_i}$, all $(\hat{u}_{ij},u_{ij})\in\R_{u_{i}},\forall j\neq i$, and $\hat u_{i}\in\Uh_i$, $\Wt_i(\cdot|\xh{i},x_i,\red{\uh{i}})$ is a sub-probability coupling  of $\hat \Tr_i(\cdot|\hat x_i,\red{\uh{i}})$ and
%		 $\Tr_i(\cdot|x_i,\red{\bar{u}_i})$, where $\red{\bar{u}_i:=[u_{i1},\ldots,u_{i(i-1)},\InF_i(\xh{i},\x{i},\hat u_i),u_{i(i+1)},\ldots]\T}$, 
%		 over $\R_{x_i}$ with respect to $\delta_i$ (see Def.~\ref{def:submeasure_lifting}),
%		\item[(c)] $\forall (\hat x_i,x_i)\in\R_{x_i}: \mathbf d_{\Y}(\hat h_i(\hat x_i),h_i(x_i)) \leq \varepsilon_i$,
%	\end{itemize}
%	then $\Mh_i$ is in an $(\varepsilon_i,\delta_i)$-SSR with $\M_i$  that is denoted as \mbox{$\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$}.
%\end{definition}
%\Oliver{Any ideas on how to make condition (b) prettier (potentially specific to $i=1,2$) are well appreciated. We don't need $\R_{u_{i}}$ I think by choosing $\hat{u}_{ij}=:{u}_{ij}$ (discretization error accounts for rest).}

%Next, we define the interconnection of two subsystems.

%\begin{definition}[Interconnection of two subsystems]\label{def:interconnection_two}
%	%	\Oliver{Replacement for Def.~4.1 in \cite{lavaei2021compositional}.}
%	Consider two gMDPs $\M_i\!=\!(\X_i,x^0_i,\U_i, \Tr_i, h_i, \Y_i)$, $i=1,2$, with an input-output configuration which can be partitioned as in \eqref{eq:input_output_partitioning}. Then, the \emph{interconnection} of the subsystems is a gMDP $\M\!=\!(\X,x^0,\U, \Tr, h, \Y)$, also denoted as $\Interc{\M_1,\M_2}$, such that $\X=[\X_{1};\X_{2}]$, $\U=[\U_{1};\U_{2}]$, $\Y=[\Y_{1};\Y_{2}]$, and $h=[h_{11};h_{22}]$, with interconnection constraints
%	\begin{align}
%		\begin{split}\label{eq:interconnection_constraints_two}
%			u_{12}&=y_{21},\; \Y_{21}\subseteq\U_{12}\\
%			u_{21}&=y_{12},\; \Y_{12}\subseteq\U_{21}.
%		\end{split}
%	\end{align}
%	The kernel and initial distribution are given as $\Tr=\Tr_{1}\Tr_2$ and $x^0=[x^0_{1};x^0_{2}]$, respectively.
%\end{definition}

\color{black}
\input{composed_system_diagram}
%\color{blue!70!black}

%In the next theorem we establish \mbox{$\Mh\preceq^{\delta}_\eps\M$}, where $\M=\Interc{\M_1,\M_2}$ and $\Mh=\Interc{\Mh_1,\Mh_2}$, by induction from $\forall i=1,2:\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$.
%
%\begin{theorem}[\bfseries Induced compositional SSR]\label{thm:comp_induction_two}
%	%	\Oliver{Replacement for Thm.~4.3 in \cite{lavaei2021compositional}.}
%	Consider two gMDPs $\M_1,\M_2$ forming an interconnected gMDP $\M\!=\!(\X,x^0,\U, \Tr, h, \Y)=\Interc{\M_1,\M_2}$. Suppose that there exist two corresponding nominal gMDPs $\Mh_1,\Mh_2$ such that for both $i=1,2$ we have $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i$ as defined in Def.~\ref{def:ssr_subsys_two}, with corresponding relations $R_{x_i}$, $\R_{u_{i}}$ and sub-probability coupling $\Wt_i$. If we have
%	\begin{align*}
%		\forall (\hat x_1, x_1)\in\R_{x_1}&: \; \left(\hat h_{12}(\hat x_1), h_{12}(x_1)\right)\in\R_{u_{2}}\\
%		\forall (\hat x_2, x_2)\in\R_{x_2}&: \; \left(\hat h_{21}(\hat x_2), h_{21}(x_2)\right)\in\R_{u_{1}},
%	\end{align*}
%	\Oliver{Is this actually what Eq.~4.6 in \cite{lavaei2021compositional} says?}
%	then $\Mh\!=\!(\Xh,\hat x^0,\U, \Trh, \hat h, \Y)=\mathscr{I}(\Mh_1,\Mh_2)$ is in an \emph{induced compositional} $(\varepsilon, \delta)$-SSR, denoted as \mbox{$\Mh\preceq^{\delta}_\eps\M$}, with $\M$ as defined in Def.~\ref{def:subsim} with a relation $\R$ given as 
%	\begin{equation*}
%		(\hat x, x)\in\R \Leftrightarrow \forall i=1,2:\; (\hat x_i, x_i)\in\R_{x_i}
%	\end{equation*}
%	where $\hat x:=[\hat x_1;\hat x_2]$, $x:=[x_1;x_2]$,
%	and $\varepsilon=\varepsilon_1+\varepsilon_2$, $\delta=1-(1-\delta_1)(1-\delta_2)$. Furthermore, we obtain the sub-probability coupling $\Wt=\Wt_{1}\Wt_2$ and the interface function $\InF=\InF_{1}\InF_2$, applying the interconnection constraints \eqref{eq:interconnection_constraints_two}.
%\end{theorem}
%\begin{proof}
%	We show that $\Mh$ is in an SSR with $\M$ by proving that the conditions in Def.~\ref{def:subsim} hold.
%	Condition (a) holds by setting the initial states $\hat x^{0} = x^{0}$. Furthermore, for all $(\hat x_1, x_1)\in\R_{x_{1}}$, $(\hat x_2, x_2)\in\R_{x_{2}}$ we have the following relation:
%	\begin{align}
%%		\begin{split}
%			&\norm{\hat h(\hat x)-h(x)}=\norm{[\hat h_{11}(\hat x);\hat h_{22}(\hat x)]-[h_{11}(x);h_{22}(x)]}\nonumber\\
%			&\hspace{20pt}\leq\norm{\hat h_{11}(\hat x_1)-h_{11}(x_1)}+\norm{\hat h_{22}(\hat x_2)-h_{22}(x_2)}\nonumber\\
%			&\hspace{20pt}\leq\norm{\hat h_{1}(\hat x_1)-h_{1}(x_1)}+\norm{\hat h_{2}(\hat x_2)-h_{2}(x_2)}.\label{eq:proof_comp_induction_two_eq}
%%		\end{split}
%	\end{align}
%	Since the individual subsystems are in a pairwise SSR as defined in Def.~\ref{def:ssr_subsys_two}, it follows from \eqref{eq:proof_comp_induction_two_eq} that $\varepsilon=\varepsilon_1+\varepsilon_2$. Hence, condition (c) of Def.~\ref{def:subsim} is satisfied.
%	
%	Finally, for all $\hat u\in\Uh$, $(\hat x,x)\in\R$, $(\hat{u}_{ij},u_{ij})\in\R_{u_{i}}\forall j\neq i$, and $\hat u_{i}\in\Uh_i$ we have
%	\begin{align*}
%		&\Wt(d\xhp\times d\xp\given \hat x,x,\hat u=[\hat u_{11},\hat u_{22}]\T) =\\
%		&\hspace{50pt}\Wt_1(d\xhp_1\times d\xp_1\given (\hat x_1,x_1)\in\R_{x_1},[\hat u_{11},\hat u_{12}]\T)\\
%		&\hspace{50pt}\times\Wt_2(d\xhp_2\times d\xp_2\given (\hat x_2,x_2)\in\R_{x_2},[\hat u_{21},\hat u_{22}]\T).
%	\end{align*}
%	Since both $\Wt_1$ and $\Wt_2$ are valid sub-probability couplings as defined in Def.~\ref{def:submeasure_lifting}, it follows that $\Wt$ is a valid sub-probability coupling as well.
%	
%	
%	Integrating over $\R$, i.e., integrating $\Wt_i$ individually over $\R_{x_i}$, yields that for all $(\hat x,x)\in\R$, $(\hat x_1,x_1)\in\R_{x_1}$, $(\hat x_2,x_2)\in\R_{x_2}$, $(\hat{u}_{ij},u_{ij})\in\R_{u_{i}}\forall j\neq i$ we have
%	\begin{align*}
%		&\int_{(\xhp, \xp)\in\R} \Wt(d\xhp\times d\xp\given \hat x,x,\hat u)=\\
%		&\hspace{50pt}\int_{(\xhp_1, \xp_1)\in\R_{x_1}} \!\!\!\!\!\!\!\! \Wt_1(d\xhp_1\times d\xp_1\given \hat x_1,x_1,[\hat u_{11},\hat u_{12}]\T)\\
%		&\hspace{50pt}\times\int_{(\xhp_2, \xp_2)\in\R_{x_2}} \!\!\!\!\!\!\!\! \Wt_2(d\xhp_2\times d\xp_2\given \hat x_2,x_2,[\hat u_{21},\hat u_{22}]\T)\\
%		&\hspace{50pt}\geq (1-\delta_1)(1-\delta_2).
%	\end{align*}
%	Hence, condition (b) is satisfied with $\delta = 1-(1-\delta_1)(1-\delta_2)$.	
%\end{proof}

\smallskip
\noindent\textbf{Linear subsystems:}
Let us now look at the case where the overall system can be decomposed into two linear subsystems. 
Consider two interconnected linear systems, $i=1,2$:
\begin{align}
	\M_i(\theta_i): \left\{ \begin{array}{ll}
		\xp_i &= A_i x_i+ B_i u_i+F_i \theta_i+ B_{w,i} w_i\\
		y_i &= C_i x_i\\
%		\iout{i} &= E_i x_i,
	\end{array} \right.\label{eq:linear_sys_subsys_two}
\end{align}
and the corresponding nominal models
\begin{align}
	\Mh_i: \left\{ \begin{array}{ll}
		\xhp_i &= A_i \hat x_i+  B_i \hat u_i+ B_{w,i}\hat w_i\\
		\hat y_i &=  C_i \hat x_i\\
%		\iouth{i} &= E_i \hat x_i.
	\end{array} \right.\label{eq:linear_nom_subsys_two}
\end{align}
The transition kernels can consequently be written as
\begin{align*}
	\Tr_i(\dxp_i \given x_i, u_i) &= \mathcal N(\dxp_i|A_i x_i+ B_i u_i+ F_i \theta_i, B_{w,i}B_{w,i}\T)\\
	\Trh_i(\dxhp_i \given \hat x_i, \hat u_i) &= \mathcal N(\dxhp_i|A_i \hat x_i+ B_i \hat u_i, B_{w,i}B_{w,i}\T).
\end{align*}

As before, assume that we can partition the input and output matrices as follows:
\begin{equation*}
	B_i=[B_{i1}, B_{i2}],\quad C_i=[C_{i1}, C_{i2}].
\end{equation*}
The matrices $\hat{B}$ and $\hat{C}$ are partitioned in a similar way.

%\hrule
We choose the interface function $\ac{i}\sim\InF_i(\cdot|\hat x_i, x_i, \hat u_i):=\ach{i}$,
and the noise coupling $\hat w_i=w_i+B_{w,i}^{-1} F_i\theta_i$ to get the state mapping
\[ \xhp_i = \xp_i-A (x_i-\hat x_i)-B(\ac{i}-\ach{i}), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_subsys_two}
	\xhp_i \sim \Refi_i(\cdot |\xh{i}, \x{i}, \xp_{i},\ach{i}) = \delta_{\xp_i-A x^\Delta_i-B u^\Delta_i}(d\xhp_i).
\end{equation}
To establish an SSR $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$, we select the relations
\begin{align}
	\R_{x_i}&:=\{ (\hat x_i,x_i)\in\Xh_i\times\X_i \given x_i=\hat x_i\}\label{eq:R_x_two}\\
	\R_{u_{i}}&:=\{ (\hat u_{ij},u_{ij})\in\Uh_{ij}\times\U_{ij} \given u_{ii}=\hat u_{ii}\}.\label{eq:R_v_two}
\end{align}
Condition (a) of Def.~\ref{def:ssr_subsys_two} holds by setting the initial states $\hat x^{0}_i = x^{0}_i$. Condition (c) is satisfied with $\eps_i=0$ since both systems use the same output mapping. For condition (b), we define the sub-probability coupling $\Wt_i$ of $\hat \Tr_i(\cdot|\hat x_i,\ach{i})$ and $\Tr_i(\cdot|x_i,\InF_i)$ over $\R_{x_i}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_subsys_two}
		\Wt_i
		&=\del{d\xhp_i}{\xp_i}
		\min\{\mathcal N(d\xp_i|\Phi_i,B_{w,i}B_{w,i}\T),\\
		&\hspace{60pt}\mathcal N(d\xp_i|\Phi_i-B_{w,i}^{-1} F_i\theta_i, B_{w,i}B_{w,i}\T)\},
	\end{split}
\end{align}
with $\Phi_i := A_i x_i+ B_i u_i+ F_i\theta_i$, that takes the minimum of two probability measures.

\begin{theorem}
	\label{thm:linear_subsys_two}
	For the linear models in \eqref{eq:linear_sys_subsys_two}-\eqref{eq:linear_nom_subsys_two}, we have that $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ with interface function $\ac{i} = \ach{i}$, relations \eqref{eq:R_x_two}-\eqref{eq:R_v_two}, and the sub-probability kernel \eqref{eq:subprobcoup_subsys_two}. The state mapping \eqref{eq:statemap_subsys_two} defines a valid control refinement with $\eps_i=0$ and
	\begin{equation}
		\label{eq:delta_subsys_two}
		\delta_i = \sup_{\theta_i\in\Theta_i}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\norm{B_{w,i}^{-1} F_i\theta_i}}\right\rbrace.
	\end{equation}
\end{theorem}
\begin{proof}
	The proof is similar to that of Thm.~\ref{thm:linear} in App.~\ref{app:proofSSRlinear}.
\end{proof}
%\begin{proof}
%	See \ref{proof:linear_subsys_two}.
%\end{proof}

\smallskip
\noindent\textbf{Composed system:}
Now, we connect two subsystems, $i\in\{1,2\}$, with $u_{12}=y_{21}$ and $u_{21}=y_{12}$ (and similarly, with $\hat u_{12}=\hat y_{21}$ and $\hat u_{21}=\hat y_{12}$). 
For $x:=[x_1,x_2]\T\in\X$, $\hat x:=[\hat x_1,\hat x_2]\T\in\Xh$, $u:=[u_1,u_2]\T\in\A$, $\hat u:=[\hat u_1,\hat u_2]\T\in\Ah$, and $\theta:=[\theta_1,\theta_2]\T\in\Theta$ we find the compositional transition kernels for the interconnected gMDPs $\M(\theta)$ and $\Mh$, namely
\begin{align*}
	\Tr(\dxp \given x, u) &= \mathcal N(\dxp|\bar A x+ B u+F \theta, B_wB_w\T)\\
	\Trh(\dxhp \given \hat x, \hat u) &= \mathcal N(\dxhp|\bar A \hat x+ B \hat u, B_wB_w\T).
\end{align*}
%with $u=\hat u$, $x=\hat x$, and 
where $B:=\mathrm{diag}(B_1,B_2)$, $F:=\mathrm{diag}(F_1,F_2)$, $B_w:=\mathrm{diag}(B_{w,1}B_{w,2})$, and
\begin{align*}
	\bar A&:=\begin{bmatrix} A_1 & B_{12}C_{21} \\ B_{21}C_{12} & A_2 \end{bmatrix}.
\end{align*}

We get the state mapping
\[ \xhp = \xp-\bar A (x-\hat x)-B (\ac{}-\ach{}), \]
not dependent on $\theta$, i.e.,
\begin{equation}
	\label{eq:statemap_comp_two}
	\xhp \sim \Refi(\cdot |\xh{}, \x{}, \xp{},\ach{}) = \delta_{\xp-\bar A x^\Delta-B u^\Delta}(d\xhp).
\end{equation}
To establish an SSR of the composed system, i.e., $\Mh\preceq^{\delta}_{\eps}\M(\theta)$, we select the relation
\begin{align}\label{eq:R_comp_two}
	\R_{x}&:=\{ (\hat x,x)\in\Xh\times\X \given x=\hat x\}
\end{align}
Condition (a) of Def.~\ref{def:subsim} holds by setting the initial states $\hat x^{0} = x^{0}$. Condition (c) is satisfied with $\eps=0$ since both compositional systems use the same output mapping $C:=\mathrm{diag}(C_1,C_2)$. For condition (b), we define the sub-probability coupling $\Wt$ of $\hat \Tr(\cdot|\hat x,\ach{})$ and $\Tr(\cdot|x,\InF)$ over $\R_{x}$:
\begin{align}
	\begin{split}\label{eq:subprobcoup_comp_two}
		\Wt&=\del{d\xhp}{\xp} \min\{\mathcal N(d\xp|\Phi,B_wB_w\T),\\
		&\hspace{100pt}\mathcal N(d\xp|\Phi-B_w^{-1}F\theta, B_wB_w\T)\},
	\end{split}
\end{align}
with $\Phi := \bar A x+ B u+ F\theta$.

Now, we want to establish a probabilistic relation after the composition using Thm.~\ref{thm:comp_induction_two}, which enables us to get guarantees on the closeness of the composed system and its abstraction using Thm.~\ref{thm:linear_subsys_two}.


\begin{theorem}\label{thm:compositional}
	Consider two pairs of linear subsystems \eqref{eq:linear_sys_subsys_two}-\eqref{eq:linear_nom_subsys_two}, where $\Mh_i\preceq^{\delta_i}_{\eps_i}\M_i(\theta_i)$ for $i=1,2$ with relations \eqref{eq:R_x_two}-\eqref{eq:R_v_two}, interface functions $u_i=\hat u_i$, and sub-probability kernels \eqref{eq:subprobcoup_subsys_two}.
	Let $\M=\Interc{\M_1,\M_2}$ and $\Mh=\Interc{\Mh_1,\Mh_2}$ be the interconnections of these linear subsystems. Then, Thm.~\ref{thm:comp_induction_two} holds, with relation $\R=\{ (\hat x,x)\in\Xh\times\X\given x=\hat x\}$, interface function $\ac{} = \ach{}$, and sub-probability kernel \eqref{eq:subprobcoup_comp_two}.
\end{theorem}
\begin{proof}
	It is trivial to show that the interconnection constraints in Thm.~\ref{thm:comp_induction_two} hold for this choice of relations $\R_{x_i},\R_{u_{i}}$.
\end{proof}

	Limitations of the compositional approach presented in this section are mainly due to the resulting cumulative $(\varepsilon,\delta)$ as in Thm.~\ref{thm:comp_induction_two}. In practice, the resulting $(\varepsilon,\delta)$ yields more conservative satisfaction probabilities than a system-holistic approach would incur. Therefore, exploiting compositionality entails trading conservative results for computational relieve. Bedsides that, for large-scale compositional systems  \red{where the individual subsystems affect each other only mildly} , switching from a dissipativity to a max small-gain approach as in \cite{Lavaei2020smallgain}, for example, may yield less conservative results, since the global $\varepsilon$ does not grow with the number of subsystems.
	
	Furthermore, designing controllers for each subsystem in isolation requires either (a) specification that can be partitioned as well or (b) all subsystems to be identical. \Oliver{Isn't this correct?!}
	
	\subsection{Proof of Theorem~\ref{thm:linear_subsys_two}}
	Similar to the proof of Thm.~\ref{thm:linear} in App.~\ref{app:proofSSRlinear}.
	
	\new{\begin{proof}[Proof (Thm.~\ref{thm:linear_subsys_two})]\label{proof:linear_subsys_two}
			\Oliver{Will be changed!!!}
			For the sub-probability coupling we have that
			\begin{align*}
				\Wt_i(d\xhp_i\times d\xp_i \given \hat x_i,x_i, \hat u_i,\hat v_i,v_i)
				&=\int_{w} \del{d\xhp_i}{A_i \hat x_i+ B_i \hat u_i+ D_i \hat v_i+ B_{w,i}(w_i+B_{w,i}^{-1} F_i\theta_i)}
				\del{d\xp_i}{A_i x_i+ B_i u_i+ D_i v_i+ B_{w,i} w_i+F_i \theta_i}\cdot\\
				&\hspace{20pt}\times\min\{\mathcal N(dw|0,I),\mathcal N(dw|-B_{w,i}^{-1} F_i\theta_i, I)\}.
			\end{align*}
			With $w_i=B_{w,i}^{-1}(\xp_i-A_ix_i-B_iu_i-D_iv_i-F_i\theta_i)$ we get
			\begin{align*}
				&\Wt_i
				=\del{d\xhp_i}{\xp_i + A_i \hat x^\Delta_i+ B_i \hat u^\Delta_i+ D_i \hat v^\Delta_i}\cdot
				\int_{w} \del{d\xp_i}{A_i x_i+ B_i u_i+ D_i v_i+ B_{w,i} w_i+F_i \theta_i}\cdot
				\min\{\mathcal N(dw|0,I),\mathcal N(dw|-B_{w,i}^{-1} F_i\theta_i, I)\},
			\end{align*}
			simplifying using $x_i=\hat x_i$, $u_i=\hat u_i$,  $v_i=C_ix_i=C_i \hat x_i=\hat v_i$
			\begin{align*}
				&\Wt_i
				=\del{d\xhp_i}{\xp_i}\cdot
				\int_{w} \del{d\xp_i}{A_i x_i+ B_i u_i+ D_i v_i+ B_{w,i} w_i+F_i \theta_i}\cdot
				\min\{\mathcal N(dw|0,I),\mathcal N(dw|-B_{w,i}^{-1} F_i\theta_i, I)\},
			\end{align*}
			and reordering, giving
			\begin{align*}
				\Wt_i
				&=\del{d\xhp_i}{\xp_i}
				\min\{\mathcal N(d\xp_i|\Phi_i,B_{w,i}B_{w,i}\T), \mathcal N(d\xp_i|\Phi_i-B_{w,i}^{-1} F_i\theta_i, B_{w,i}B_{w,i}\T)\},
			\end{align*}
			with $\Phi_i := A_i x_i+ B_i u_i+ D_i v_i+ F_i\theta_i$.
			
			Then, the following state mapping defines a valid control refinement with $\eps_i=0$ and 
			\begin{equation*}
				\delta_i = \sup_{\theta_i\in\Theta_i}\left\lbrace  1 - 2\cdot\cdf{-\frac{1}{2}\norm{B_{w,i}^{-1} F_i\theta_i}}\right\rbrace,
			\end{equation*}
			namely
			\begin{align*}
				\xhp_i &= \xp_i + ( A_i \hat x_i+  B_i \hat u_i+  D_i \hat v_i)  - (A_i x_i+ B_i u_i+ D_i v_i+F_i \theta_i) + F_i\theta_i
				= \xp_i - A_i x^\Delta_i- B_i u^\Delta_i- D_i v^\Delta_i,
			\end{align*}
			where $x^\Delta_i:= x_i-\hat x_i$, $u^\Delta_i:= u_i-\hat u_i$, and $v^\Delta_i:= v_i-\hat v_i$.
	\end{proof}}
	
	\bigskip

==> simrel_subsys.tex <==
% !TEX root = main.tex
\begin{figure}
	\centering
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
		%uncomment if require: \path (0,216); %set diagram left start at 0, and has height of 216
		
		%% System 1
		%Rounded Rect [id:dp22217799131680738] 
		\draw  [fill=grayfilling] (40,51) .. controls (40,44.92) and (44.92,40) .. (51,40) -- (84,40) .. controls (90.08,40) and (95,44.92) .. (95,51) -- (95,84) .. controls (95,90.08) and (90.08,95) .. (84,95) -- (51,95) .. controls (44.92,95) and (40,90.08) .. (40,84) -- cycle ;
		% Freeform cutout
%		\draw  plot[smooth, tension=.7] coordinates {(0, 80) (0, 55) (30, 15) (68, 0) (135, 55)};
		%Straight Lines [id:da08273469517536802] 
		\draw    (0,55) -- (38,55) ;
		\draw [shift={(40,55)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da7286474312267406] 
		\draw    (0,80) -- (31,80) -- (37.5,80) ;
		\draw [shift={(39.5,80)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da8497687026000231] 
		\draw    (68.5,0) -- (68.5,38) ;
		\draw [shift={(68.5,40)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da4118975490556376] 
		\draw    (0,80) -- (0,135) ;
		%Straight Lines [id:da8937728440260815] 
		\draw    (134.5,80) -- (135,135) ;
		%Straight Lines [id:da8764463118163162] 
		\draw    (95,55) -- (133,55) ;
		\draw [shift={(135,55)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
		%Straight Lines [id:da9345959359825047] 
		\draw    (95,80) -- (126,80) -- (134.5,80) ;
		
		
		%% System 2
		
		
		
		
		% Text Node
		\draw (55.5+1,57.4+2.5+1) node [anchor=north west][inner sep=0.75pt]    {$\M_{1}$};
		% Text Node
		\draw (45+1,8.4+2.5) node [anchor=north west][inner sep=0.75pt]    {$w_{1}$};
		% Text Node
		\draw (2+1,58.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{12}$};
		% Text Node
		\draw (2+1,33.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{11}$};
		% Text Node
		\draw (97+1,58.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{12}$};
		% Text Node
		\draw (97+1,33.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{11}$};
		% Text Node
%		\draw (13+1,138.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{22}$};
%		% Text Node
%		\draw (13+1,113.4+10) node [anchor=north west][inner sep=0.75pt]    {$y_{21}$};
%		% Text Node
%		\draw (108+1,138.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{22}$};
%		% Text Node
%		\draw (108+1,113.4+10) node [anchor=north west][inner sep=0.75pt]    {$u_{21}$};
%		% Text Node
%		\draw (45+1,189.4+2.5) node [anchor=north west][inner sep=0.75pt]    {$w_{2}$};
%		% Text Node
%		\draw (55.5+1,137.4+2.5+1) node [anchor=north west][inner sep=0.75pt]    {$\M_{2}$};
		
		% Freeform cutout
%		\draw  plot[smooth, tension=.7] coordinates {(-3.5,0.5) (-3,2.5) (-1,3.5) (1.5,3) (4,3.5) (5,2.5) (5,0.5) (2.5,-2) (0,-0.5) (-3,-2) (-3.5,0.5)};
	\end{tikzpicture}
	\caption{...}
	\label{fig:simrel_subsys}
\end{figure}
